GPWM: Modeling the World as 3D Particle Motion

We introduce GPWM, a Generative Particle World Model that predicts how 3D scenes evolve by generating the motion of particles and rigid bodies over time. Unlike video world models that generate scene appearance, GPWM operates directly in 3D physical space. A single representation and architecture cover rigid, deformable, cloth, and granular materials, in both passive physics and robotic interaction. GPWM is an object-aware multi-resolution transformer that combines flow matching with diffusion forcing to generate coherent physical trajectories far beyond its training horizon. We train and evaluate GPWM on ParticleWorlds, a 25.5-million-frame corpus spanning diverse geometries, materials, interactions, and robot embodiments. GPWM outperforms the best prior learned-dynamics baseline in each of six physical domains, reducing prediction error by 31% on average. Breaking from the domain-specific setting of prior methods, a single Unified GPWM models these heterogeneous regimes with one set of weights, largely outperforming per-domain baselines and even surpassing our own specialist models in two domains. GPWM further generalizes to unseen geometries, physical properties, object counts, and rollout horizons. Beyond prediction, GPWM enables contact-rich planning by learning a generative prior over joint actuator-object motion. Instead of searching over unconstrained actions, planning searches the model's latent noise for interactions that achieve a desired object-space goal. With the same world model, noise-space planning substantially outperforms action-space search on pushing and picking, where complex contact sequences are hard to discover. Executed open-loop in simulation, the resulting plans achieve goal-directed manipulation without reference action trajectories or goal-specific policies.

==> macros.tex <==



\newcommand{\pendingresult}{--}
\RequirePackage{tikz}
\definecolor{gpwmA}{HTML}{0284C7}
\definecolor{gpwmB}{HTML}{9333EA}
\makeatletter
\newsavebox{\gpwm@box}
\ifdefined\pdfliteral
  \newcommand{\gpwm@name}{\sbox{\gpwm@box}{\pdfliteral direct{7 Tr}GPWM}\tikz[baseline=0pt]\path[left color=gpwmA,right color=gpwmB]\pgfextra{\rlap{\usebox{\gpwm@box}}}(0,-\dp\gpwm@box) rectangle (\wd\gpwm@box,\ht\gpwm@box);}
\else
  \newcommand{\gpwm@name}{{\color{gpwmA}G\color{gpwmB!33!gpwmA}P\color{gpwmB!67!gpwmA}W\color{gpwmB}M}}
\fi
\DeclareRobustCommand{\gpwmgradient}{\gpwm@name}
\newcommand{\model}{GPWM}
\makeatother
\AtBeginDocument{\ifdefined\pdfstringdefDisableCommands\pdfstringdefDisableCommands{\def\gpwmgradient{GPWM}}\fi}
\providecommand{\dataset}{\textsc{ParticleWorlds}}



